Multi-Agent Reinforcement Learning with Shared Resources for Inventory Management

In this paper, we consider the inventory management (IM) problem where we need to make replenishment decisions for a large number of stock keeping units (SKUs) to balance their supply and demand. In our setting, the constraint on the shared resources (such as the inventory capacity) couples the otherwise independent control for each SKU. We formulate the problem with this structure as Shared-Resource Stochastic Game (SRSG)and propose an efficient algorithm called Context-aware Decentralized PPO (CD-PPO). Through extensive experiments, we demonstrate that CD-PPO can accelerate the learning procedure compared with standard MARL algorithms.

==> src/app_local_simulator.tex <==
Our algorithm follows a decentralized training paradigm, which is compatible with distributed training framework. We can run parallel local simulation while communication cost of context dynamics is also acceptable. With distributed training, our method can be much more efficient than learning from the joint simulator directly. 

One may argue that we can also learn from joint simulator efficiently by implementing a distributed/parallelized joint simulator. While this can indeed improve sampling efficiency in many scenarios, its usefulness is limited particularly for systems with a large number of agents. In a typical multi-agent system, interactions occur frequently among all agents. Actually, one advantage of multi-agent systems is to model complex interactions among agents. However, such interactions will remarkably reduce the efficiency improvement brought by parallelism, as these interactions often require involved agents to synchronize which usually consumes lots of time on waiting and communicating. For instance, in IM problems, at each time step, all agents should be synchronized in order to calculate $\rho$ in Eq.~\ref{eq:rho} before moving to the next time step. 

On the other hand, in our local sampling approach we simplify such costly interactions by utilizing special structures of shared-resource stochastic games. Under our approach, there is no need for agents to be synchronized before moving to the next time step in local simulators. As a result, our method can be much more efficient than learning only from the joint simulator in practice. 

==> src/app_related_work.tex <==
\subsection{Training Paradigm in MARL}
In this section we will provide a more detailed description of related work for training paradigm used in MARL.
From the perspective of training schemes, it can be devided into three categories: decentralized training decentralized execution (DTDE), centralized training centralized execution (CTCE) and centralized training decentralized execution (CTDE). Recent deep MARL works often use the CTDE or CTCE training pradigm.\\

The CTCE paradigm allows the straightforward employment of single-agent approaches such as Actor-Critic~\citep{mnih2016asynchronous} or policy gradient algorithms~\citep{schulman2017proximal} to multi-agent problems. The representative work of CTCE is~\citep{gupta2017cooperative}, which represented the centralized executor as a set of independent sub-policies such that agents’ individual action distributions are captured rather than the joint action distribution of all agents.\\
\quad \quad Value-based CTDE approaches, which are also known as Value Decomposition methods~\citep{peng2020facmac,mahajan2019maven,rashid2020weighted,rashid2018qmix,son2019qtran,sunehag2017value,wang2020roma,wang2019learning}, mianly focus on how centrally learned value functions can be reasonably decoupled into decentralized ones and have shown promising results. Policy-gradient-based methods on CTDE, on the other hand, have heavily relied on centralized critics. One of the first works utilizating a centralized critic was COMA~\citep{foerster2018counterfactual}, a framework adopting a centralized critic with a counterfactual baseline. For convergence properties, COMA establishes that the overall effect on decentralized policy gradient with a centralized critic can be reduced to a single-agent actor-critic approach, which ensures convergence under the similar assumptions like A2C. \\

Concurrently with COMA, MADDPG~\citep{lowe2017multi} proposed to use a dedicated centralized critic for each agent in semi-competitive domains, demonstrating compelling empirical results in continuous action environments. 
Recently, MAPPO~\citep{yu2021surprising}, an on-policy policy gradient multi-agent reinforcement learning algorithm, achieves strong results comparable to the state-of-the-art on a variety of cooperative multi-agent challenges. Despite its on-policy nature, MAPPO is competitive to ubiquitous off-policy methods such as MADDPG, QMix, and RODE in terms of final performance, and in the vast majority of cases, comparable to off-policy methods in terms of sample-efficiency.
In addition, many incremental research inspired by MADDPG, COMA or MAPPO also borrowed the centralized critic baselines e.g. M3DDPG~\citep{li2019robust}, SQDDPG~\citep{wang2020shapley}, etc. Mean Filed Q-Learning~\citep{pmlr-v80-yang18d,carmona2019modelfree} takes a different approach from the CTDE based methods. It employs mean field approximation over the joint action space in order to address the scalability issue that exists in the prior methods.\\

Contrary to CTDE, in DTDE paradigm, each agent has an associated policy which maps local observations to a distribution over individual actions. No information is shared between agents such that each agent learns independently. DTDE has been applied to cooperative navigation task~\citep{chen2017decentralized,strouse2018learning}, to partially observable domains~\citep{dobbe2017fully,srinivasan2018actor}, and to social dilemmas~\citep{leibo2017multi}. For more comparisons of centralized critic and decentralized critic, please see~\citep{lyu2021contrasting}.\\

In this paper, we design a decentralized traning paradigm avoiding the flaws of traditional training paradigms proposed in literature. The fundamental drawback of the DTDE paradigm is that the environment appears non-stationary from a single agent's viewpoint because agents neither have access to the knowledge of others, nor do they perceive the joint action. Some studies reported that DTDE scale poorly with the number of agent due to the extra sample complexity, which is added to the learning problem~\citep{gupta2017cooperative}; An obvious flaw for CTDE/CTCE is that state-action  spaces grow exponentially by the number of agents. Even though there are some attempts proposed that the joint model can be factored into individual policies for each agent To address the so-called curse of dimensionality, CTDE/CTCE methods have to use at least joint states overall agents as the input to approximate global value function to give guidance for centralized critics or decentralized policies. Meaning that these traditional training schemes still not have strong expansion capabilities to large number of agents when system's state is combined by local state for each agent. As for our approach, we train agents independently with learned dynamics model of utilization's trend for shared resource, which will give agent enough information to learn optimal policy. At the meantime, we can also, improve efficiency of data sampling since we don't always use the original joint simulator containing all agents for data collection. Instead, we mainly running the light-cost local simulator by embedding the learned dynamic model, which can significantly reduce the cost of data collection process, especially when running joint simulator (such as inventory management) expensively. 

\subsection{MDP Scenarios in MARL}
There are limited similar variants of MDP settings which have been studied under MARL framework, to our knowledge. Dec-POMDP~\citep{oliehoek2016concise} is the most common setting studied in MARL research, especially in fully cooperative tasks in which agents share the global team reward rather than individual rewards; In the scenarios of Constrained MDP setting (C-MDP, \citep{bhatnagar2012online,wang2019learning,diddigi2019actor}), there are some constraints in the system, such as the penalty caused by illegal actions in autonomous driving~\citep{zhang2016decision,fowler2018constrained}, the resource-allocation constraints in scheduling tasks~\citep{agrawal2016scalable,dolgov2006resource}, or limited bandwidth during communicating among agents~\citep{fowler2018constrained}, etc. Similar with C-MDP, Weakly-Coupled Constrained MDP (WC-C-MDP \citep{boutilier2016budget}) consider the problem of budget (or other resource) allocation in sequential decision problems involving a large number of concurrently running sub-processes,whose only interaction is through their consumption of budget. 
Different from mentioned scenarios, we focus on the situation where agents can only get the individual reward from the environment, so that team reward is invisible; Comparing with C-MDP and WC-C-MDP, the penalty of overstocking in which is related with stock levels of all agents in future, while in C-MDP and WC-C-MDP, the corresponding cost function is only based on historical states of the system. Leading that we can not optimize only the combined objective of long-term summation of return and penalty.

\subsection{Model-Based MARL}

For model-based MARL, there are relatively limited works of literature. P-MARL~\citep{marinescu2015p} proposed an approach that integrates prediction and pattern change detection abilities into MARL and thus minimises the effect of non-stationarity in the environment. The environment is modelled as a time-series, with future estimates provided using prediction techniques. Learning is based on the predicted environment behaviour, with agents employing this knowledge to improve their performance in real-time. \citep{park2019multi} proposed to use a centralized auxiliary prediction network to model the environment dynamics to alleviate the non-stationary dynamics problem. \citep{krupnik2020multi} built a centralized multi-step generative model with a disentangled variational auto-encoder to predict the environment dynamics and the opponent actions and then performed trajectory planning. AORPO~\citep{zhang2021model} is a Dyna-style method in which each agent builds its multi-agent environment model that consist of a dynamics model and multiple opponent models, and trains its policy with the data both generated from adaptive opponent-wise rollout and interacted from the real environment. To our knowledge, unlike previous work, our approach is the first to accelerate the learning process in MARL by building only a part dynamic model of the whole system. Our algorithm is also a Dyna-style method like AORPO. And it is clear that the difficulty of modeling process will be reduced significantly and the learning process is more efficient.  
